Implicit Filter Sparsification In Convolutional Neural Networks

We show implicit filter level sparsity manifests in convolutional neural networks (CNNs) which employ Batch Normalization and ReLU activation, and are trained with adaptive gradient descent techniques and L2 regularization or weight decay. Through an extensive empirical study (Mehta et al., 2019) we hypothesize the mechanism behind the sparsification process, and find surprising links to certain filter sparsification heuristics proposed in literature. Emergence of, and the subsequent pruning of selective features is observed to be one of the contributing mechanisms, leading to feature sparsity at par or better than certain explicit sparsification / pruning approaches. In this workshop article we summarize our findings, and point out corollaries of selective-featurepenalization which could also be employed as heuristics for filter pruning

==> Tables/imagenet_basic.tex <==
%%!TEX root = ../article.tex
\renewcommand{\tabcolsep}{1.5pt}
%\begin{table}[h!]
\centering
\caption{Convolutional filter sparsity of BasicNet on ImageNet.}
\label{tbl:imagenet_basic}
\resizebox{0.80\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c}
                       & Batch & Train                       & Val                         & Top 1    & Top 5    & \% Sparsity \\
                       & Size  & Loss                        & Loss                        & Val Err. & Val Err. & by $\gamma$ \\ \hline
                       & 64    & {\color[HTML]{9B9B9B} 2.05} & {\color[HTML]{9B9B9B} 1.58} & 38.0     & 15.9     & 0.2          \\
                       & 256    & {\color[HTML]{9B9B9B} 1.63} & {\color[HTML]{9B9B9B} 1.35} & 32.9     & 12.5     & 0.0          \\
\end{tabular}
}
%\end{table}

==> Tables/layerwise_sparsity_cifar10.tex <==
%%!TEX root = ../supp_article.tex
\renewcommand{\tabcolsep}{1.5pt}
%\begin{table*}[]
%\begin{table*}[!htbp]
\centering
\caption{Layerwise \% filters pruned from BasicNet trained on CIFAR10, based on the $|\gamma| <10^{-3}$ criteria. Also shown are pre-pruning and post-pruning test error, and the \% of \emph{convolutional} parameters pruned. C1-C7 indicate Convolution layer 1-7, and the numbers in parantheses indicate the total number of features per layer. Average of 3 runs. Also see Table 2 in the main document.}
\label{tbl:layerwise_sparsity_cifar10}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lcccccccccccccc}
                    \multicolumn{2}{l}{\textbf{CIFAR10}}                                & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}           & \multicolumn{1}{l|}{}          & \multicolumn{8}{c|}{\% Sparsity by $\gamma$ or \% Filters Pruned}                                                                                                                                                                & \multicolumn{1}{l|}{\% Param}                                          & \multicolumn{1}{l}{}         \\ \cline{6-13}
                       & \multicolumn{1}{l|}{}         &    Train                  & \multicolumn{1}{c|}{Test}          & \multicolumn{1}{c|}{Test}          & C1                   & C2                   & C3                   & C4                   & C5                   & C6                   & \multicolumn{1}{c|}{C7}    & \multicolumn{1}{c|}{Total}  & \multicolumn{1}{c|}{Pruned}                                            & Pruned                       \\
               & \multicolumn{1}{l|}{}         & Loss           & \multicolumn{1}{c|}{Loss} & \multicolumn{1}{c|}{Err}  & (64)                 & (128)                & (128)                & (256)                & (256)                & (512)                & \multicolumn{1}{c|}{(512)} & \multicolumn{1}{c|}{(1856)} & \multicolumn{1}{c|}{(4649664)}                                           & Test Err.                    \\ \hline
\multicolumn{1}{|c}{}                       & \multicolumn{1}{|c|}{L2: 1e-3} & 0.29                 & \multicolumn{1}{c|}{0.41}      & \multicolumn{1}{c|}{13.1}      & 59                   & 57                   & 42                   & 74                   & 76                   & 97                   & \multicolumn{1}{c|}{98}    & \multicolumn{1}{c|}{83}     & \multicolumn{1}{c|}{97}                        & 13.5 \\
\multicolumn{1}{|c}{}                       & \multicolumn{1}{|c|}{L2: 1e-4} & 0.06                 & \multicolumn{1}{c|}{0.43}      & \multicolumn{1}{c|}{10.5}      & 44                   & 22                   & 6                    & 45                   & 54                   & 96                   & \multicolumn{1}{c|}{95}    & \multicolumn{1}{c|}{70}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 90}} & 10.5 \\ \cline{2-15} 
\multicolumn{1}{|c}{}                       & \multicolumn{1}{|c|}{WD: 2e-4} & 0.22                 & \multicolumn{1}{c|}{0.42}      & \multicolumn{1}{c|}{13.4}      & 57                   & 27                    & 9                    & 19                    & 46                   & 77                   & \multicolumn{1}{c|}{91}    & \multicolumn{1}{c|}{60}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 83}} & 13.4 \\
\multicolumn{1}{|c}{\multirow{-4}{*}{\rotatebox[origin=c]{90}{Adam \B}}} & \multicolumn{1}{|c|}{WD: 1e-4} & 0.07                 & \multicolumn{1}{c|}{0.42}      & \multicolumn{1}{c|}{11.2}      & 45                    & 4                    & 0                    & 0                    & 14                    & 51                    & \multicolumn{1}{c|}{78}     & \multicolumn{1}{c|}{40}      & \multicolumn{1}{c|}{63}                         & 11.2 \\ \hline
\multicolumn{1}{|c}{}                       & \multicolumn{1}{|c|}{L2: 1e-3} & 0.62                 & \multicolumn{1}{c|}{0.64}      & \multicolumn{1}{c|}{21.8}      & 86                   & 61                   & 53                   & 46                   & 65                   & 4                    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{27}     & \multicolumn{1}{c|}{38}                                                & 21.8                         \\
\multicolumn{1}{|c}{}                       & \multicolumn{1}{|c|}{L2: 5e-4} & 0.38                 & \multicolumn{1}{c|}{0.49}      & \multicolumn{1}{c|}{16.3}      & 68                    & 16                    & 9                    & 9                    & 24                    & 0                    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{9}      & \multicolumn{1}{c|}{13}                         & 16.5 \\ \cline{2-15} 
\multicolumn{1}{|c}{}                       & \multicolumn{1}{|c|}{WD: 1e-3} & 0.61                 & \multicolumn{1}{c|}{0.63}      & \multicolumn{1}{c|}{21.6}      & 85                   & 60                   & 51                   & 46                   & 66                   & 4                   & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{27}     & \multicolumn{1}{c|}{{\color[HTML]{000000}38}} & 21.6 \\
\multicolumn{1}{|c}{\multirow{-4}{*}{\rotatebox[origin=c]{90}{SGD}}}  & \multicolumn{1}{|c|}{WD: 5e-4} & 0.38                 & \multicolumn{1}{c|}{0.46}      & \multicolumn{1}{c|}{15.8}      & 69                    & 19                    & 7                    & 7                    & 23                    & 0                    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{8}      & \multicolumn{1}{c|}{13}                         & 16.1 \\ \hline
                                            & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}                                                   & \multicolumn{1}{l}{}         \\
\end{tabular}
}
%\end{table*}

==> Tables/layerwise_sparsity_cifar100.tex <==
%%!TEX root = ../article.tex
\renewcommand{\tabcolsep}{1.5pt}
%\begin{table*}[]
\begin{table*}[]
\centering
\caption{Layerwise \% filters pruned from BasicNet trained on CIFAR100, based on the $|\gamma| <10^{-3}$ criteria. Also shown are pre-pruning and post-pruning test error, and the \% of \emph{convolutional} parameters pruned. C1-C7 indicate Convolution layer 1-7, and the numbers in parantheses indicate the total number of features per layer. Average of 3 runs. Color and highlighting indicates high and low sparsity for best and near best test errors, as in Table~\ref{tbl:all_optim}.}
\label{tbl:layerwise_sparsity}
\resizebox{0.70\linewidth}{!}{
\begin{tabular}{lcccccccccccccc}
                                             \multicolumn{2}{l}{}          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}           & \multicolumn{1}{l|}{}          & \multicolumn{8}{c|}{\% Sparsity by $\gamma$ or \% Filters Pruned}                                                                                                                                                                & \multicolumn{1}{l|}{\% Param}                                          & \multicolumn{1}{l}{}         \\ \cline{6-13}
                       & \multicolumn{1}{l|}{}         &    Train                  & \multicolumn{1}{c|}{Test}          & \multicolumn{1}{c|}{Test}          & C1                   & C2                   & C3                   & C4                   & C5                   & C6                   & \multicolumn{1}{c|}{C7}    & \multicolumn{1}{c|}{Total}  & \multicolumn{1}{c|}{Pruned}                                            & Pruned                       \\
               & \multicolumn{1}{l|}{}         & Loss           & \multicolumn{1}{c|}{Loss} & \multicolumn{1}{c|}{Err}  & (64)                 & (128)                & (128)                & (256)                & (256)                & (512)                & \multicolumn{1}{c|}{(512)} & \multicolumn{1}{c|}{(1856)} & \multicolumn{1}{c|}{(4649664)}                                           & Test Err.                    \\ \hline
\multicolumn{1}{|l}{}                       & \multicolumn{1}{|c|}{L2: 1e-3} & 1.06                 & \multicolumn{1}{c|}{1.41}      & \multicolumn{1}{c|}{39.0}      & 56                   & 47                   & 43                   & 68                   & 72                   & 91                   & \multicolumn{1}{c|}{85}    & \multicolumn{1}{c|}{76}     & \multicolumn{1}{c|}{95}                        & 39.3 \\
\multicolumn{1}{|l}{}                       & \multicolumn{1}{|c|}{L2: 1e-4} & 0.10                 & \multicolumn{1}{c|}{1.98}      & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}36.6}      & {\color[HTML]{009901}41}                   & {\color[HTML]{009901}20}                   & {\color[HTML]{9A0000}9}                    & {\color[HTML]{009901}33}                   & {\color[HTML]{009901}34}                   & {\color[HTML]{009901}67}                   & \multicolumn{1}{c|}{\color[HTML]{009901}55}    & \multicolumn{1}{c|}{\color[HTML]{009901}47}     & \multicolumn{1}{c|}{\color[HTML]{009901}74}                        & \cellcolor[HTML]{9AFF99}36.6 \\ \cline{2-15} 
\multicolumn{1}{|l}{}  & \multicolumn{1}{|c|}{WD: 2e-4} & 0.34                 & \multicolumn{1}{c|}{1.56}      & \multicolumn{1}{c|}{37.3}      & \color[HTML]{009901}55                    & \color[HTML]{009901}20                    & \color[HTML]{9a0000}3                    & \color[HTML]{9a0000}4                    & \color[HTML]{9a0000}2                    & \color[HTML]{009901}16                    & \multicolumn{1}{c|}{\color[HTML]{009901}26}     & \multicolumn{1}{c|}{\color[HTML]{009901}16}      & \multicolumn{1}{c|}{\color[HTML]{009901}27}                                                 & 37.3                         \\ 
\multicolumn{1}{|c}{\multirow{-4}{*}{\rotatebox[origin=c]{90}{Adam}}} & \multicolumn{1}{|c|}{WD: 1e-4} & 0.08                 & \multicolumn{1}{c|}{1.76}      & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}36.2}      & {\color[HTML]{009901}38}                   & {\color[HTML]{9a0000}4}                    & {\color[HTML]{9a0000}0}                    & {\color[HTML]{9a0000}0}                    & {\color[HTML]{9a0000}0}                    & {\color[HTML]{9a0000}0}                    & \multicolumn{1}{c|}{\color[HTML]{9a0000}5}     & \multicolumn{1}{c|}{\color[HTML]{9A0000}3}      & \multicolumn{1}{c|}{\color[HTML]{9a0000}4}                                                 & {\cellcolor[HTML]{9AFF99}36.2}                        \\ \hline
%\multicolumn{1}{|l}{}                       & \multicolumn{1}{|c|}{L2: 1e-3} & 1.49                 & \multicolumn{1}{c|}{1.78}      & \multicolumn{1}{c|}{47.1}      & 82                   & 41                   & 33                   & 29                   & 33                   & 6                    & \multicolumn{1}{c|}{18}    & \multicolumn{1}{c|}{23}     & \multicolumn{1}{c|}{34}                        & 47.1 \\
%\multicolumn{1}{|l}{}                       & \multicolumn{1}{|c|}{L2: 5e-4} & 0.89                 & \multicolumn{1}{c|}{1.69}      & \multicolumn{1}{c|}{42.1}      & 64                    & 3                    & 3                    & 3                    & 2                    & 0                    & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{4}      & \multicolumn{1}{c|}{4}                         & 42.1 \\ \cline{2-15} 
%\multicolumn{1}{|l}{}                       & \multicolumn{1}{|c|}{WD: 1e-3} & 1.49                 & \multicolumn{1}{c|}{1.79}      & \multicolumn{1}{c|}{47.6}      & 82                   & 43                   & 31                   & 28                   & 33                   & 6                   & \multicolumn{1}{c|}{17}    & \multicolumn{1}{c|}{23}     & \multicolumn{1}{c|}{34}                                                & 47.6                         \\
%\multicolumn{1}{|c}{\multirow{-4}{*}{\rotatebox[origin=c]{90}{SGD}}}  & \multicolumn{1}{|c|}{WD: 5e-4} & 0.89                 & \multicolumn{1}{c|}{1.69}      & \multicolumn{1}{c|}{41.9}      & 66                    & 2                    & 1                   & 4                    & 2                    & 0                    & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{4}      & \multicolumn{1}{c|}{4}                         & 41.9 \\ \hline
\end{tabular}
}
\vspace{-0.2cm}
\end{table*}

==> Tables/layerwise_sparsity_cifar100_scale_bias.tex <==
%%!TEX root = ../supp_article.tex
\renewcommand{\tabcolsep}{1.5pt}
%\begin{table*}[]
\begin{table*}[]
\centering
\caption{Layerwise \% filters pruned from BasicNet trained on CIFAR100, based on the $|\gamma| <10^{-3}$ criteria. Also shown are pre-pruning and post-pruning test error. C1-C7 indicate Convolution layer 1-7, and the numbers in parantheses indicate the total number of features per layer. We analyse the effect of different initializations of $\beta$s, as well as the effect of different relative learning rates for $\gamma$s and $\beta$s, when trained with Adam with L2 regularization of $10^{-4}$. Average of 3 runs.}
%\kimki{I guess we do not need to use resize box for the tables that are smaller than the column or row width.}}
\label{tbl:layerwise_sparsity_cifar100_scale_bias}
\begin{tabular}{ccccccccccccc}
\\
                                             \multicolumn{4}{l|}{\textbf{}}             & \multicolumn{8}{c|}{\% Sparsity by $\gamma$ or \% Filters Pruned}                                                                                                                                                                &                                            \multicolumn{1}{l}{}         \\ \cline{5-12}
                        \multicolumn{1}{l|}{}         &    Train                  & \multicolumn{1}{c|}{Test}          & \multicolumn{1}{c|}{Test}          & \T C1                   & C2                   & C3                   & C4                   & C5                   & C6                   & \multicolumn{1}{c|}{C7}    & \multicolumn{1}{c|}{Total}                                               & Pruned                       \\
                \multicolumn{1}{l|}{}         & Loss           & \multicolumn{1}{c|}{Loss} & \multicolumn{1}{c|}{Err}  & (64)                 & (128)                & (128)                & (256)                & (256)                & (512)                & \multicolumn{1}{c|}{(512)} & \multicolumn{1}{c|}{(1856)}                                            & Test Err.                    \\ \hline
 \multicolumn{1}{c|}{Baseline ($\gamma_{init}$=1, $\beta_{init}$=0)} & 0.10                 & \multicolumn{1}{c|}{1.98}      & \multicolumn{1}{c|}{36.6}      & 41                   & 20                   & 9                    & 33                   & 34                   & 67                   & \multicolumn{1}{c|}{55}    & \multicolumn{1}{c|}{46}                            & \T 36.6 \\ \hline 
 \multicolumn{1}{c|}{$\gamma_{init}$=1, $\beta_{init}$=$-$0.1} & 0.10                 & \multicolumn{1}{c|}{1.98}      & \multicolumn{1}{c|}{37.2}      & 44                   & 20                   & 10                    & 34                   & 32                   & 68                   & \multicolumn{1}{c|}{54}    & \multicolumn{1}{c|}{46}                            & \T 36.5 \\ \hline 
 \multicolumn{1}{c|}{$\gamma_{init}$=1, $\beta_{init}$=1.0} & 0.14                 & \multicolumn{1}{c|}{2.04}      & \multicolumn{1}{c|}{38.4}      & 47                   & 29                   & 25                    & 36                   & 46                   & 69                   & \multicolumn{1}{c|}{61}    & \multicolumn{1}{c|}{53}                            & \T 38.4 \\ \hline 
 \multicolumn{13}{l}{Different Learning Rate Scaling for $\beta$ and $\gamma$} \\ \hline
 \multicolumn{1}{c|}{LR scale for $\gamma$: 0.1} & 0.08                 & \multicolumn{1}{c|}{1.90}      & \multicolumn{1}{c|}{35.0}      & 16                   & 6                   & 1                    & 13                   & 20                   & 52                   & \multicolumn{1}{c|}{49}    & \multicolumn{1}{c|}{33}                            & \T 35.0 \\ \hline 
 \multicolumn{1}{c|}{LR scale for $\beta$: 0.1} & 0.12                 & \multicolumn{1}{c|}{1.98}      & \multicolumn{1}{c|}{37.1}      & 42                   & 26                   & 21                    & 41                   & 48                  & 70                   & \multicolumn{1}{c|}{55}    & \multicolumn{1}{c|}{51}                            & \T 37.1 \\ \hline 
\end{tabular}
%}
\vspace{-0.3cm}
\end{table*}

==> Tables/net_width.tex <==
%%!TEX root = ../article.tex
\renewcommand{\tabcolsep}{1.5pt}
%\begin{table}[h!]
\centering
\caption{Effect of varying the number of features in BasicNet. }
\begin{tabular}{c|cccc|c|cccc}
         & \multicolumn{4}{c}{CIFAR 10}                                                                                                                  &  & \multicolumn{4}{c}{CIFAR 100}                                                                                                                 \\ \cline{2-10} 
Net      & \multicolumn{1}{c|}{Train}                       & \multicolumn{1}{c|}{Test}                        & \multicolumn{1}{c|}{Test} & \%Spar.  &  & \multicolumn{1}{c|}{Train}                       & \multicolumn{1}{c|}{Test}                        & \multicolumn{1}{c|}{Test} & \%Spar.  \\
Cfg.     & \multicolumn{1}{c|}{Loss}                        & \multicolumn{1}{c|}{Loss}                        & \multicolumn{1}{c|}{Err}  & by $\gamma$ &  & \multicolumn{1}{c|}{Loss}                        & \multicolumn{1}{c|}{Loss}                        & \multicolumn{1}{c|}{Err}  & by $\gamma$ \\ \hline
64-1x    & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 0.06}} & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 0.43}} & \multicolumn{1}{c|}{10.5} & 70          &  & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 0.10}} & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 1.98}} & \multicolumn{1}{c|}{36.6} & 46          \\
64-0.5x  & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 0.10}} & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 0.41}} & \multicolumn{1}{c|}{11.0} & 51          &  & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 0.11}} & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 2.19}} & \multicolumn{1}{c|}{39.8} & 10          \\
32-0.25x & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 0.22}} & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 0.44}} & \multicolumn{1}{c|}{13.4} & 23          &  & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 0.51}} & \multicolumn{1}{c|}{{\color[HTML]{9B9B9B} 2.05}} & \multicolumn{1}{c|}{43.4} & 0           \\ \hline
\end{tabular}
%\end{table}

==> Tables/vgg16_imagenet.tex <==
%%!TEX root = ../article.tex
\renewcommand{\tabcolsep}{2.5pt}
%\begin{table}[h!]
\centering
\caption{Sparsity observed on VGG-16, trained on ImageNet. Network structure as in ~\cite{simonyan2014very} with BatchNorm}
\label{tbl:vgg16_imagenet}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|cc|c|c|}
                &        \# Conv               & \multicolumn{2}{c|}{Pre-pruning}    & \multicolumn{2}{c|}{Post-pruning} \\
                &  Feat. Pruned & \multicolumn{1}{c|}{top1}  & top5  & top1          & top5        \\ \hline
Adam, L2: 1e-4, B: 40 & 292           & \multicolumn{1}{c|}{29.93} & 10.41 & 29.91         &     10.41       \\
\end{tabular}
}
%\end{table}
